GSC-QEMit: A Telemetry-Driven Hierarchical Forecast-and-Bandit Framework for Adaptive Quantum Error Mitigation

Quantum error mitigation (QEM) is essential for extracting reliable results from near-term quantum devices, yet practical deployments must balance mitigation strength against runtime overhead under time-varying noise. We introduce \emph{GSC-QEMit}, a telemetry-driven, \textbf{context--forecast--bandit} framework for \emph{adaptive} mitigation that switches between lightweight suppression and heavier intervention as drift evolves. GSC-QEMit composes three coupled modules: (G) a Growing Hierarchical Self-Organizing Map (GHSOM) that clusters streaming telemetry into operating contexts; (S) an uncertainty-aware subsampled Gaussian-process forecaster that predicts short-horizon fidelity degradation; and (C) a cost-aware contextual multi-armed bandit (CMAB) that selects mitigation actions via Thompson sampling with explicit intervention cost. We evaluate GSC-QEMit on benchmark circuit families (GHZ, Quantum Fourier Transform, and Grover search) under nonstationary noise regimes simulated in Qiskit Aer, using an instrumented testbed where action labels correspond to graded mitigation intensity. Across Clifford, non-Clifford, and structured workloads, GSC-QEMit improves average logical fidelity by \textbf{+9.0\%} relative to unmitigated execution while reducing unnecessary heavy interventions by reserving them for inferred noise spikes. The resulting policies exhibit a favorable fidelity--cost trade-off and transfer across the evaluated workloads without circuit-specific tuning.

==> New_Sections/simulator_breakdown.tex <==
\subsection{Qiskit-Based Repetition-Code Simulator}
\label{subsec:qiskit-simulator}

We evaluate our controller on a Qiskit Aer backend that implements a repetition-style memory for a single logical bit under time-varying bit-flip noise. The backend supports code distances $d \in \{1,3,5\}$; in our main experiments we use $d=5$. The aim is not to reproduce a specific circuit-level decoder, but to provide a nonstationary testbed in which different QEC/QEM action labels induce different logical-error--versus--cost trade-offs under a common telemetry interface.

At control cycle $t \in \{0,1,\dots,T-1\}$ we define a base bit-flip rate
\begin{equation}
\begin{aligned}
  \mathrm{frac}_t &= \frac{t \bmod T}{T},\\
  p_{\mathrm{base}}(t)
  &= \operatorname{clip}\bigl(
       p_{\mathrm{phys}0}\,[1 + 0.5 \sin(2\pi\,\mathrm{frac}_t)],
       10^{-4}, 0.5
     \bigr),
\end{aligned}
\label{eq:p-base}
\end{equation}
where $p_{\mathrm{phys}0}$ is a nominal physical error rate, $T$ a drift period, and $\operatorname{clip}(x,a,b) = \min(\max(x,a),b)$. This sinusoidal drift sweeps through cleaner and noisier regimes within a single episode.

Each control action is a label $\ell \in \mathcal{A}$ interpreted as a QEC/QEM strategy. We model these strategies as surrogates that rescale the instantaneous bit-flip rate and incur different abstract costs: a scaling factor $s(\ell) \in \{1.0, 0.9, 0.7, 0.5, 0.3\}$ defines an effective rate
\begin{equation}
  p_{\mathrm{eff}}(t,\ell)
  = \operatorname{clip}\bigl(
      s(\ell)\,p_{\mathrm{base}}(t), 10^{-5}, 0.5
    \bigr).
  \label{eq:p-eff}
\end{equation}
More aggressive labels have smaller $s(\ell)$ and thus lower $p_{\mathrm{eff}}$. These factors stand in for classes of interventions (e.g., higher-distance codes, more expensive decoders, postselection); the controller only observes logical-error and cost signals, so the same interface could be connected to more realistic implementations.

At each cycle a logical bit $b_t \in \{0,1\}$ is drawn uniformly and encoded as
\begin{equation}
  |b_t\rangle_{\mathrm{L}}
  =
  |b_t\rangle^{\otimes d}
  =
  U_{\mathrm{enc}} \, |b_t\rangle,
\end{equation}
by applying an $X$ on qubit $0$ if $b_t=1$ and CNOTs from qubit $0$ to the remaining $d-1$ qubits. Bit-flip noise is injected using Qiskit Aer’s \texttt{NoiseModel} via an independent Pauli-$X$ channel on each qubit,
\[
  \mathcal{E}_{\mathrm{BF}}(\rho)
  =
  (1 - p_{\mathrm{eff}})\,\rho
  + p_{\mathrm{eff}}\, X \rho X,
\]
with overall map $\mathcal{E}_{\mathrm{BF}}^{\otimes d}$. The encoded state before measurement on cycle $t$ is
\begin{equation}
  \rho_t
  =
  \bigl(\mathcal{E}_{\mathrm{BF}}^{\otimes d} \circ U_{\mathrm{enc}}\bigr)
  \bigl(|b_t\rangle\!\langle b_t|\bigr).
\end{equation}

We then measure all $d$ qubits for $N = \texttt{shots}$ repetitions, yielding bitstrings $\mathbf{x}^{(j)}$. Majority decoding produces $\hat b_t^{(j)}$ and a detection flag $\delta_{\mathrm{det}}^{(j)}$. The per-cycle detection rate, logical error rate, and logical fidelity are
\begin{equation}
  \hat p_{\mathrm{det}}(t)
  =
  \frac{1}{N} \sum_{j=1}^N \delta_{\mathrm{det}}^{(j)},
  \qquad
  \hat \varepsilon_{\mathrm{logical}}(t)
  =
  \frac{1}{N} \sum_{j=1}^N
  \mathbb{I}[\hat b_t^{(j)} \neq b_t],
\end{equation}
\begin{equation}
  F_{\mathrm{logical}}(t)
  =
  1 - \hat \varepsilon_{\mathrm{logical}}(t).
\end{equation}
All statistics, together with additional QDataset-style telemetry features~\cite{perrier2022qdataset}, form the per-cycle observation.

Using Qiskit Aer as the plant follows standard practice in QEC and quantum-architecture studies~\cite{quantumsim}. Our backend implements a small repetition code with a configurable time-varying bit-flip channel and computes the same observables that underpin recent below-threshold surface-code experiments on devices such as Google’s Willow processor: logical error per cycle $\varepsilon_d$, logical fidelity $F_{\mathrm{logical}} \approx 1 - \varepsilon_d$, and distance-scaling factors $\Lambda(d_1 \to d_2) = \varepsilon_{d_1}/\varepsilon_{d_2}$~\cite{google2025quantum}. Although our code is much smaller than a full surface code, expressing results in these metrics makes the simulations qualitatively comparable to larger threshold studies while providing a minimal, analytically transparent testbed for our context--forecast--bandit controller.

